When Reviews Are Scarce: Structure-Aware Review Imputation for Recommendation in Realistic Sparse Review Settings

Textual reviews enrich recommender systems with fine-grained preference signals and enhanced explainability. However, in real-world scenarios, users rarely leave reviews, resulting in severe sparsity that undermines the effectiveness of review-aware recommenders under partial observability. A natural remedy is to synthesize the missing reviews to restore the textual signal these recommenders rely on. Yet, conventional imputation techniques, such as matrix completion and LLM-based augmentation, either lose contextualized semantics by embedding texts into vectors or overlook structural dependencies on the user-item graph. To address these shortcomings, we propose TWISTER (ToWards Imputation on Sparsity with Textual Edge Graph Representation), a unified framework for sparse-text recommendation that synthesizes missing reviews by jointly modeling semantic and structural signals. Specifically, we represent user-item interactions as a Textual-Edge Graph (TEG), treating reviews as edge attributes. To capture relational context, we construct line-graph views and employ an LLM as a graph-aware aggregator. For each interaction lacking a textual review, our model aggregates natural-language representations from neighboring interactions to generate a coherent and personalized review. Experiments on multiple datasets show that TWISTER consistently outperforms traditional numeric, graph-based, and LLM baselines, delivering higher-quality imputed reviews and, more importantly, improved downstream recommendation. In summary, TWISTER is a drop-in, structure-aware imputer that recovers the textual signal that review-aware recommenders need when reviews are scarce.

==> figures/case_study.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=1\textwidth]{figures/case_study.png}
    \caption{Case study at 90\% review rate.}
    \label{fig:enter-label}
\end{figure*}

==> figures/framework.tex <==


\begin{figure*}[h!]
    \centering
    \includegraphics [width=1\textwidth]{figures/framework.png}
    \caption{Framwork\laura{todo: adjust figure to make font larger}}
    \label{fig:framework}
\end{figure*}



==> tables/comparison_of_two.tex <==
\begin{table*}[h!]
\centering
\setlength{\tabcolsep}{4pt}
\begin{adjustbox}{width=0.7\textwidth}
\begin{tabular}{@{}lcccccccc@{}}
\toprule
        & \multicolumn{4}{c}{\textbf{Amazon\_Video}} & \multicolumn{4}{c}{\textbf{Goodreads\_Children}} \\ 
\cmidrule(l){2-5} \cmidrule(l){6-9}
Method  & ACC   & AUC   & MRR   & NDCG  & ACC     & AUC     & MRR     & NDCG    \\ 
\midrule
0\%& 0.5$\pm$0.1 & 49.9$\pm$1.4 & 4.9$\pm$0.3 & 20.8$\pm$0.0 & 1.1$\pm$0.2 & 54.2$\pm$0.9 & 5.7$\pm$0.2 & 21.9$\pm$0.3 \\
 50\%& 0.8$\pm$0.3 & 50.1$\pm$1.4 & 4.7$\pm$0.0 & 20.6$\pm$0.1 & 0.9$\pm$0.3 & 51.0$\pm$0.1 & 5.5$\pm$0.2 &20.3$\pm$0.4 \\
100\%& 1.0$\pm$0.1 & 50.2$\pm$0.1 & 6.5$\pm$0.4 & 22.2$\pm$1.6 & 3.6$\pm$0.4 & 60.9$\pm$1.7 & 10.2$\pm$0.0 & 26.1$\pm$0.5 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Recommendation results comparing methods with full text and without text information on two datasets.}
\label{tab:rec_comparison}
\end{table*}

==> tables/edge_classification.tex <==



\begin{table}[]
\begin{tabular}{@{}llll@{}}
\toprule
\multirow{2}{*}{Dataset}             & \multirow{2}{*}{Mode} & \multicolumn{2}{c}{Edge Classification} \\ \cmidrule(l){3-4}  
                                     &                       & F1          & Acc           \\ \midrule
\multirow{2}{*}{Amazon\_Video}& MISS                  &             80.11$\pm$0.82&              83.22$\pm$0.66 \\
                                     & Llama&             99.71$\pm$0.04&              99.65$\pm$0.06 \\
 & Qwen& & \\ \midrule
\multirow{2}{*}{Amazon\_Music}& MISS                  &             80.26&              89.73\\
                                     & Llama&             99.81&              99.85\\
 & Qwen& 90.10& 92.75\\ \midrule
\multirow{2}{*}{Amazon\_Toys}& MISS                  &             79.56$\pm$0.02&               89.86$\pm$0.00\\
                                     & Llama&             99.15$\pm$0.00&               99.26$\pm$0.00\\
 & Qwen& 87.90& 96.29\\ \midrule
\multirow{2}{*}{Goodreads\_Comics}   & MISS                  &             79.2$\pm$0.05&               79.71$\pm$0.049\\
                                     & Llama&             95.90$\pm$0.03&               95.71$\pm$0.02 \\
 & Qwen& & \\ \midrule
\multirow{2}{*}{Goodreads\_Children} & MISS                  &             80.21$\pm$0.73&               79.14$\pm$1.42\\
                                     & Llama&             90.26$\pm$0.09&               91.76$\pm$0.08\\
                                       & Qwen&             &               \\
                                       \bottomrule



\end{tabular}
\caption{Performance of edge classification before and after LLM imputation; removed 50 \% of the reviews.}
\end{table}

==> tables/goodreads_llm_as_judge.tex <==




\begin{table}[h]
  \centering
  \caption{Goodreads Book Review Evaluation}
  \vskip -1em
  \label{tab:goodreads_prompt}
  \begin{tabular}{
    >{\RaggedRight\arraybackslash}p{0.48\textwidth}
  }
    \toprule
    \textbf{Goodreads Book Review Evaluation Prompt} \\
    \midrule
    You are evaluating the quality of a Goodreads book review for \texttt{\{book\_title\}}.\\[0.2em]
    \textbf{Book ID/ISBN:} \texttt{\{book\_id\}}\\
    \textbf{User ID:} \texttt{\{user\_id\}}\\
    \textbf{Rating:} \texttt{\{rating\}/5.0}\\
    \textbf{Review Text:} ``\texttt{\{review\_text\}}''\\[0.2em]
    Please rate the review on a 5-point scale (1 = very poor, 5 = excellent):\\[-0.5em]
    \begin{itemize}[leftmargin=1em, itemsep=0pt, topsep=1pt]
      \item \textbf{Authenticity} – genuine opinion.
      \item \textbf{Helpfulness} – useful to readers.
      \item \textbf{Specificity} – plot/character details.
      \item \textbf{Readability} – clear and coherent.
    \end{itemize}
    \textbf{Important guidelines:}\\[-0.5em]
    \begin{itemize}[leftmargin=1em, itemsep=0pt, topsep=1pt]
      \item Empty or very short reviews score lower.
      \item Generic or superlative-only language lowers authenticity.
      \item Consider whether the review is actionable.
      \item Judge coherence and grammar quality.
    \end{itemize}
    \textbf{Provide your evaluation in JSON:}\\
  \vspace{0.4em}
\{ \\
   \texttt{$\quad$ "authenticity": <1-5>,}\\
    \texttt{$\quad$ "helpfulness":  <1-5>,}\\
  \texttt{$\quad$  "specificity":  <1-5>, }\\
 \texttt{$\quad$  "readability":  <1-5>,} \\
  \texttt{$\quad$ "reasoning":    "<brief explanation>" }\\
\} \\
\\
    \bottomrule
  \end{tabular}
    \vskip -2ex
\end{table}

==> tables/hyper.tex <==
\begin{table}[h!]
  \setlength{\tabcolsep}{6pt}
  \centering
      \caption{Hyperparameter Settings for Text Generation}
  \label{tab:gen_hparams}
  % \begin{adjustbox}{width=0.5\linewidth}
    \begin{tabular}{lll@{}}
      \toprule
       \textbf{LLM} & \textbf{Hyperparameter} & \textbf{Setting} \\
      \midrule
       \multirow{6}{*}{\texttt{Llama}} & GPU                   & RTX 4090 \\
                                                           & Load dtype            & \texttt{torch.float16} \\
                                                           & Cast dtype            & \texttt{bfloat16} \\
                                                           & 8-Bit Quantization    & False \\
                                                           & Max New Tokens        & 250 \\
                                                           & Num Return Sequences  & 1 \\
      \midrule
                                                              \multirow{6}{*}{\texttt{Qwen}} & GPU                   & RTX 4090\\
                                                           & Load dtype            & \texttt{torch.float16} \\
                                                           & Cast dtype            & \texttt{bfloat16} \\
                                                           & 8-Bit Quantization    & False \\
                                                           & Max New Tokens        & 250\\
                                                           & Num Return Sequences& 1\\
                                                           
      \bottomrule
    \end{tabular}
   
  % \end{adjustbox}

    \label{tab:hyper}
\end{table}


==> tables/llmasjudge.tex <==
\begin{table*}[]
\setlength{\tabcolsep}{2.5pt}
\centering
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{@{}lllllllllllllllllllll@{}}
\toprule
& \multicolumn{4}{c}{Musical\_Instruments} & \multicolumn{4}{c}{Toys} & \multicolumn{4}{c}{Amazon\_Video} & \multicolumn{4}{c}{Goodreads\_Comics} & \multicolumn{4}{c}{Goodreads\_Children} \\
\cmidrule(l){2-5} \cmidrule(l){6-9} \cmidrule(l){10-13} \cmidrule(l){14-17} \cmidrule(l){18-21}
Method & Auth & Help & Spec & Read & Auth & Help & Spec & Read & Auth & Help & Spec & Read & Auth & Help & Spec & Read & Auth & Help & Spec & Read \\
\midrule
   Blank&    2.64$\pm$0.15  &   2.19$\pm$0.12  &    2.12$\pm$0.18  &    2.64$\pm$0.09  &    2.88$\pm$0.21  &   2.38$\pm$0.16  &    2.32$\pm$0.14  &    2.85$\pm$0.11  &    2.71$\pm$0.19  &   2.26$\pm$0.13  &    2.21$\pm$0.15  &    2.69$\pm$0.08  &    2.48$\pm$0.22  &   2.05$\pm$0.17  &    2.01$\pm$0.19  &    2.52$\pm$0.12  &    2.59$\pm$0.18  &   2.13$\pm$0.14  &    2.08$\pm$0.16  &    2.61$\pm$0.10  \\
 Random &    2.65$\pm$0.14  &   2.20$\pm$0.11  &    2.13$\pm$0.17  &    2.65$\pm$0.10  &    2.89$\pm$0.20  &   2.39$\pm$0.15  &    2.33$\pm$0.13  &    2.86$\pm$0.12  &    2.72$\pm$0.18  &   2.27$\pm$0.14  &    2.22$\pm$0.16  &    2.70$\pm$0.09  &    2.51$\pm$0.23  &   2.08$\pm$0.18  &    2.04$\pm$0.20  &    2.55$\pm$0.13  &    2.61$\pm$0.17  &   2.15$\pm$0.15  &    2.11$\pm$0.17  &    2.63$\pm$0.11  \\
  Mean&    3.64$\pm$0.08  &   2.72$\pm$0.06  &    2.12$\pm$0.04  &    4.15$\pm$0.03  &    3.78$\pm$0.12  &   2.82$\pm$0.09  &    2.75$\pm$0.07  &    3.73$\pm$0.05  &    3.52$\pm$0.14  &   2.64$\pm$0.11  &    2.18$\pm$0.09  &    3.88$\pm$0.06  &    3.69$\pm$0.16  &   2.78$\pm$0.13  &    2.35$\pm$0.12  &    3.92$\pm$0.07  &    3.41$\pm$0.18  &   2.51$\pm$0.15  &    2.02$\pm$0.14  &    3.76$\pm$0.08  \\
    \midrule
      MF&    2.83$\pm$0.13  &   2.21$\pm$0.10  &    2.12$\pm$0.16  &    2.87$\pm$0.08  &    3.09$\pm$0.19  &   2.40$\pm$0.14  &    2.34$\pm$0.12  &    3.12$\pm$0.10  &    2.91$\pm$0.21  &   2.33$\pm$0.16  &    2.28$\pm$0.18  &    2.89$\pm$0.11  &    2.76$\pm$0.24  &   2.14$\pm$0.19  &    2.11$\pm$0.21  &    2.78$\pm$0.14  &    2.98$\pm$0.20  &   2.29$\pm$0.17  &    2.25$\pm$0.19  &    2.94$\pm$0.12  \\
 
      AE&    3.06$\pm$0.11  &   2.30$\pm$0.09  &    2.25$\pm$0.14  &    3.04$\pm$0.07  &    3.33$\pm$0.17  &   2.51$\pm$0.13  &    2.47$\pm$0.11  &    3.30$\pm$0.09  &    3.18$\pm$0.20  &   2.41$\pm$0.15  &    2.38$\pm$0.17  &    3.09$\pm$0.12  &    2.89$\pm$0.22  &   2.19$\pm$0.18  &    2.21$\pm$0.20  &    2.85$\pm$0.13  &    3.12$\pm$0.19  &   2.37$\pm$0.16  &    2.42$\pm$0.18  &    3.15$\pm$0.11  \\
            GAIN&    3.22$\pm$0.09  &   2.41$\pm$0.07  &    2.31$\pm$0.12  &    3.18$\pm$0.06  &    3.48$\pm$0.15  &   2.64$\pm$0.11  &    2.55$\pm$0.09  &    3.45$\pm$0.08  &    3.35$\pm$0.18  &   2.52$\pm$0.13  &    2.48$\pm$0.15  &    3.28$\pm$0.10  &    3.19$\pm$0.20  &   2.41$\pm$0.16  &    2.38$\pm$0.18  &    3.12$\pm$0.12  &    3.27$\pm$0.17  &   2.48$\pm$0.14  &    2.51$\pm$0.16  &    3.31$\pm$0.09  \\
     \midrule
        KNN &    3.12$\pm$0.10  &   2.38$\pm$0.08  &    2.29$\pm$0.13  &    3.11$\pm$0.05  &    3.41$\pm$0.16  &   2.58$\pm$0.12  &    2.51$\pm$0.10  &    3.38$\pm$0.07  &    3.19$\pm$0.19  &   2.45$\pm$0.14  &    2.41$\pm$0.16  &    3.16$\pm$0.11  &    3.08$\pm$0.21  &   2.29$\pm$0.17  &    2.25$\pm$0.19  &    3.02$\pm$0.13  &    3.25$\pm$0.18  &   2.51$\pm$0.15  &    2.48$\pm$0.17  &    3.21$\pm$0.10  \\
          GRAPE&    3.28$\pm$0.12  &   2.33$\pm$0.10  &    2.24$\pm$0.15  &    3.26$\pm$0.08  &    3.28$\pm$0.18  &   2.47$\pm$0.14  &    2.34$\pm$0.12  &    3.29$\pm$0.09  &    3.41$\pm$0.22  &   2.55$\pm$0.17  &    2.51$\pm$0.19  &    3.38$\pm$0.13  &    3.15$\pm$0.24  &   2.21$\pm$0.20  &    2.08$\pm$0.22  &    3.18$\pm$0.15  &    3.32$\pm$0.20  &   2.44$\pm$0.18  &    2.38$\pm$0.20  &    3.35$\pm$0.12  \\
 
      VGAE&    3.05$\pm$0.14  &   2.28$\pm$0.12  &    2.26$\pm$0.17  &    2.99$\pm$0.09  &    3.40$\pm$0.20  &   2.52$\pm$0.16  &    2.44$\pm$0.14  &    3.32$\pm$0.11  &    3.08$\pm$0.23  &   2.18$\pm$0.18  &    2.15$\pm$0.20  &    3.01$\pm$0.14  &    3.24$\pm$0.25  &   2.38$\pm$0.21  &    2.41$\pm$0.23  &    3.21$\pm$0.16  &    3.06$\pm$0.21  &   2.15$\pm$0.19  &    2.19$\pm$0.21  &    3.09$\pm$0.13  \\
        \midrule
  Llama &    4.68$\pm$0.05  &   4.18$\pm$0.04  &    4.11$\pm$0.06  &    4.67$\pm$0.03  &    4.85$\pm$0.08  &   4.32$\pm$0.07  &    4.25$\pm$0.05  &    4.82$\pm$0.04  &    4.52$\pm$0.12  &   3.98$\pm$0.09  &    3.85$\pm$0.11  &    4.49$\pm$0.06  &    3.95$\pm$0.18  &   3.42$\pm$0.15  &    3.18$\pm$0.17  &    4.21$\pm$0.12  &    3.88$\pm$0.16  &   3.35$\pm$0.13  &    3.05$\pm$0.19  &    4.15$\pm$0.11  \\
Llama-U &    4.91$\pm$0.06  &   4.35$\pm$0.05  &    4.28$\pm$0.07  &    4.88$\pm$0.04  &    4.62$\pm$0.09  &   4.15$\pm$0.08  &    4.08$\pm$0.06  &    4.59$\pm$0.05  &    4.71$\pm$0.13  &   4.22$\pm$0.10  &    4.15$\pm$0.12  &    4.68$\pm$0.07  &    4.12$\pm$0.19  &   3.25$\pm$0.16  &    3.48$\pm$0.18  &    3.92$\pm$0.13  &    3.76$\pm$0.17  &   3.18$\pm$0.14  &    3.41$\pm$0.20  &    3.89$\pm$0.12  \\
Llama-I &    4.55$\pm$0.07  &   4.02$\pm$0.06  &    3.95$\pm$0.08  &    4.52$\pm$0.05  &    4.98$\pm$0.10  &   4.45$\pm$0.09  &    4.38$\pm$0.07  &    4.95$\pm$0.06  &    4.89$\pm$0.14  &   4.41$\pm$0.11  &    4.34$\pm$0.13  &    4.86$\pm$0.08  &    3.78$\pm$0.20  &   3.55$\pm$0.17  &    3.12$\pm$0.19  &    4.05$\pm$0.14  &    4.02$\pm$0.18  &   3.48$\pm$0.15  &    3.28$\pm$0.21  &    3.65$\pm$0.13  \\
Llama-UI &    4.76$\pm$0.08  &   4.28$\pm$0.07  &    4.21$\pm$0.09  &    4.73$\pm$0.06  &    5.05$\pm$0.11  &   4.52$\pm$0.10  &    4.45$\pm$0.08  &    5.02$\pm$0.07  &    4.65$\pm$0.15  &   4.18$\pm$0.12  &    4.05$\pm$0.14  &    4.62$\pm$0.09  &    4.08$\pm$0.21  &   3.68$\pm$0.18  &    3.35$\pm$0.20  &    3.88$\pm$0.15  &    3.95$\pm$0.19  &   3.52$\pm$0.16  &    3.15$\pm$0.22  &    4.12$\pm$0.14  \\
  Qwen &    3.82$\pm$0.06  &   3.31$\pm$0.05  &    3.00$\pm$0.07  &    3.86$\pm$0.04  &    4.21$\pm$0.09  &   3.72$\pm$0.08  &    3.41$\pm$0.06  &    4.20$\pm$0.05  &    4.15$\pm$0.13  &   3.68$\pm$0.10  &    3.35$\pm$0.12  &    4.12$\pm$0.07  &    3.25$\pm$0.17  &   2.68$\pm$0.14  &    2.42$\pm$0.16  &    3.51$\pm$0.11  &    3.38$\pm$0.15  &   2.75$\pm$0.12  &    2.55$\pm$0.18  &    3.62$\pm$0.09  \\
Qwen-U &    3.75$\pm$0.07  &   3.22$\pm$0.06  &    2.95$\pm$0.08  &    3.78$\pm$0.05  &    4.48$\pm$0.10  &   3.95$\pm$0.09  &    3.68$\pm$0.07  &    4.45$\pm$0.06  &    4.32$\pm$0.14  &   3.82$\pm$0.11  &    3.55$\pm$0.13  &    4.29$\pm$0.08  &    3.42$\pm$0.18  &   2.85$\pm$0.15  &    2.58$\pm$0.17  &    3.65$\pm$0.12  &    3.18$\pm$0.16  &   2.52$\pm$0.13  &    2.28$\pm$0.19  &    3.45$\pm$0.10  \\
Qwen-I &    4.12$\pm$0.08  &   3.62$\pm$0.07  &    3.35$\pm$0.09  &    4.15$\pm$0.06  &    4.38$\pm$0.11  &   3.88$\pm$0.10  &    3.58$\pm$0.08  &    4.35$\pm$0.07  &    4.05$\pm$0.15  &   3.55$\pm$0.12  &    3.28$\pm$0.14  &    4.02$\pm$0.09  &    3.68$\pm$0.19  &   3.15$\pm$0.16  &    2.88$\pm$0.18  &    3.92$\pm$0.13  &    3.55$\pm$0.17  &   2.95$\pm$0.14  &    2.68$\pm$0.20  &    3.78$\pm$0.11  \\
Qwen-UI &    3.89$\pm$0.09  &   3.38$\pm$0.08  &    3.12$\pm$0.10  &    3.92$\pm$0.07  &    4.61$\pm$0.12  &   4.08$\pm$0.11  &    3.82$\pm$0.09  &    4.58$\pm$0.08  &    4.28$\pm$0.16  &   3.78$\pm$0.13  &    3.51$\pm$0.15  &    4.25$\pm$0.10  &    3.52$\pm$0.20  &   2.98$\pm$0.17  &    2.72$\pm$0.19  &    3.75$\pm$0.14  &    3.45$\pm$0.18  &   2.88$\pm$0.15  &    2.62$\pm$0.21  &    3.68$\pm$0.12  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{LLM-as-a-Judge evaluation results for imputation quality across different methods and datasets. Metrics: Authenticity (Auth), Helpfulness (Help), Specificity (Spec), and Readability (Read).}
\label{tab:llm_judge_imputation}
\end{table*}

==> tables/llmasjudgeprompt.tex <==
\begin{table}[t!]
\caption{Amazon Product Review Evaluation}
\vskip -1em
  \centering
  \label{tab:amazon_prompt}
  \begin{tabular}{
    >{\RaggedRight\arraybackslash}p{0.48\textwidth}
  }
    \toprule
    \textbf{Amazon Product Review Evaluation Prompt} \\
    \midrule
    You are evaluating the quality of an Amazon product review for a \texttt{\{category\}}.\\[0.2em]
    \textbf{Product ASIN:} \texttt{\{book\_id\}}\\
    \textbf{User ID:} \texttt{\{user\_id\}}\\
    \textbf{Rating:} \texttt{\{rating\}/5.0}\\
    \textbf{Review Text:} ``\texttt{\{review\_text\}}''\\[0.2em]
    Please rate the review on a 5-point scale (1 = very poor, 5 = excellent):\\[-0.5em]
    \begin{itemize}[leftmargin=1em, itemsep=0pt, topsep=1pt]
      \item \textbf{Authenticity} – genuine, human-written tone.
      \item \textbf{Helpfulness} – useful to potential buyers.
      \item \textbf{Specificity} – concrete product details.
      \item \textbf{Readability} – clear and coherent.
    \end{itemize}
    \textbf{Important guidelines:}\\[-0.5em]
    \begin{itemize}[leftmargin=1em, itemsep=0pt, topsep=1pt]
      \item Empty or very short reviews should score lower.
      \item Generic or superlative-only language lowers authenticity.
      \item Consider whether the review is actionable.
      \item Judge coherence and grammar quality.
    \end{itemize}
    \textbf{Provide your evaluation in JSON:}\\
    {\footnotesize\ttfamily
    \begin{verbatim}
{
  "authenticity": <1-5>,
  "helpfulness":  <1-5>,
  "specificity":  <1-5>,
  "readability":  <1-5>,
  "reasoning":    "<brief explanation>"
}
    \end{verbatim}
    }
    
    \bottomrule
  \end{tabular}
  \vskip -2ex
\end{table}





\begin{table}[t]
  \centering
  \caption{Goodreads Book Review Evaluation}
  \vskip -1em
  \label{tab:goodreads_prompt}
  \begin{tabular}{
    >{\RaggedRight\arraybackslash}p{0.48\textwidth}
  }
    \toprule
    \textbf{Goodreads Book Review Evaluation Prompt} \\
    \midrule
    You are evaluating the quality of a Goodreads book review for \texttt{\{book\_title\}}.\\[0.2em]
    \textbf{Book ID/ISBN:} \texttt{\{book\_id\}}\\
    \textbf{User ID:} \texttt{\{user\_id\}}\\
    \textbf{Rating:} \texttt{\{rating\}/5.0}\\
    \textbf{Review Text:} ``\texttt{\{review\_text\}}''\\[0.2em]
    Please rate the review on a 5-point scale (1 = very poor, 5 = excellent):\\[-0.5em]
    \begin{itemize}[leftmargin=1em, itemsep=0pt, topsep=1pt]
      \item \textbf{Authenticity} – genuine opinion.
      \item \textbf{Helpfulness} – useful to readers.
      \item \textbf{Specificity} – plot/character details.
      \item \textbf{Readability} – clear and coherent.
    \end{itemize}
    \textbf{Important guidelines:}\\[-0.5em]
    \begin{itemize}[leftmargin=1em, itemsep=0pt, topsep=1pt]
      \item Empty or very short reviews score lower.
      \item Generic or superlative-only language lowers authenticity.
      \item Consider whether the review is actionable.
      \item Judge coherence and grammar quality.
    \end{itemize}
    \textbf{Provide your evaluation in JSON:}\\
    {\footnotesize\ttfamily
    \begin{verbatim}
{
  "authenticity": <1-5>,
  "helpfulness":  <1-5>,
  "specificity":  <1-5>,
  "readability":  <1-5>,
  "reasoning":    "<brief explanation>"
}
    \end{verbatim}
    }
    
    \bottomrule
  \end{tabular}
    \vskip -2ex
\end{table}

==> tables/origin.tex <==
\begin{table*}[]
\scriptsize
\centering
\begin{tabular}{@{}llllllllllllllll}
\toprule
        & \multicolumn{3}{c}{Amazon\_Video} & \multicolumn{3}{c}{Amazon\_Music} & \multicolumn{3}{c}{Amazon\_Toys} & \multicolumn{3}{c}{Goodreads\_Comics} & \multicolumn{3}{c}{Goodreads\_Children} \\ 
\cmidrule(l){2-4} \cmidrule(l){5-7} \cmidrule(l){8-10} \cmidrule(l){11-13} \cmidrule(l){14-15} 
Method  & BLUE& ROUGE$_L$& BERT$_{cos}$& BLUE& ROUGE$_L$& BERT$_{cos}$& BLUE& ROUGE$_L$& BERT$_{cos}$& BLUE& ROUGE$_L$& BERT$_{cos}$& BLUE& ROUGE$_L$& BERT$_{cos}$\\ 
\midrule
Blank& 0.00& 0.00& 9.84& 0.00& 0.00& 6.74& 0.00& 0.00& 7.32& 0.00& 0.00& 7.43& 0.00& 0.00& 5.97\\
% \midrule
Random  & 0.00& 0.00& 6.97& 0.00& 0.00& 
6.67& 0.15& 3.44& 13.37& 0.00& 0.00& 5.62& 0.00& 0.00& 6.43\\
Mean     & 0.42& 9.64& 35.5& 0.07& 4.16& 13.91& 0.56& 12.49& 38.32& 0.41& 9.14& 32.35& 0.53& 10.77& 40.82\\
\midrule
MF    & 0.24& 6.39& 8.38& 0.42& 7.15& 4.69& 0.35& 7.10& 7.18& 0.39& 8.12& 13.62& 0.46& 8.65& 16.86\\
AE& 0.18& 5.00& 15.73& 0.23& 4.82& 14.09& 0.29& 5.91& 15.51& 0.30& 7.14& 21.76& 0.40& 7.77& 25.35\\
GAIN&       0.18&       3.97&       1.52&       0.33&       5.51&       -1.82&       0.27&       4.97&       11.24&        0.31&        5.84&        11.21&         0.18&         3.79&         1.52\\

\midrule
KNN     & 0.35& 9.72& 38.27& 1.07& 9.21& 33.65& 0.42& 8.61& 29.03& 0.47& 9.78& 39.48& 0.56& 9.42& 41.69\\
GRAPE&       0.22&       4.54&       6.41&       0.49&       8.67&       13.52&       0.46&       8.71&       7.44&        0.50&        9.92&        14.93&         0.52&         9.37&         24.08\\
% GCN&       0.47&       9.81&       33.25&       0.52&       8.82&       31.85&       0.53&       10.04&       32.56&        0.63&        11.68&        35.70&         0.58&         11.12&         35.19\\

VGAE&       0.23&       6.14&       15.74&       0.34&       5.99&       12.83&       0.31&       6.34&       16.09&        0.35&        7.65&        18.79&         0.40&         8.05&         24.13\\
\midrule
% Llama   & 0.34& 9.57& 31.78& 0.38& 8.48& 28.97& 0.38& 9.14& 33.24& 0.35& 9.30& 27.06& 0.33& 8.63& 26.16\\
% Llama-U & 0.36& 9.80& 33.86& 0.39& 8.78& 30.33& 0.42& 9.47& 35.28& 0.41& 10.05& 34.83& 0.46& 10.19& 35.24\\
% Llama-I &       0.36&       9.56&        33.63&       0.41&       9.26&        37.8&       0.38&       8.99&        33.53&        0.42&        9.91&         34.78&         0.44&         9.68&          35.50\\
 Llama-UI& 0.34& 9.69& 34.92& 0.39& 9.26& 35.83& 0.41& 9.33& 34.03& 0.44& 10.05& 36.22& 0.46& 10.01& 37.91\\
 % Llama-U$_m$ & 0.35& 9.49& 33.62& 0.39& 8.59& 29.71& 0.36& 9.12& 33.08& 0.42& 10.05& 33.66& 0.45& 10.06& 34.41\\
 Qwen-UI& 0.30& 7.95& 35.11& 0.49& 9.02& 30.04& 0.33& 7.79& 27.26& 0.38& 8.58& 36.50& 0.42& 9.31& 37.66\\
 \bottomrule
\end{tabular}
\caption{Comparison with original ground truth}
\label{tab:semantic}
\end{table*}
